Flow Factorized Representation Learning

A prominent goal of representation learning research is to achieve representations which are factorized in a useful manner with respect to the ground truth factors of variation. The fields of disentangled and equivariant representation learning have approached this ideal from a range of complimentary perspectives; however, to date, most approaches have proven to either be ill-specified or insufficiently flexible to effectively separate all realistic factors of interest in a learned latent space. In this work, we propose an alternative viewpoint on such structured representation learning which we call Flow Factorized Representation Learning, and demonstrate it to learn both more efficient and more usefully structured representations than existing frameworks. Specifically, we introduce a generative model which specifies a distinct set of latent probability paths that define different input transformations. Each latent flow is generated by the gradient field of a learned potential following dynamic optimal transport. Our novel setup brings new understandings to both \textit{disentanglement} and \textit{equivariance}. We show that our model achieves higher likelihoods on standard representation learning benchmarks while simultaneously being closer to approximately equivariant models. Furthermore, we demonstrate that the transformations learned by our model are flexibly composable and can also extrapolate to new data, implying a degree of robustness and generalizability approaching the ultimate goal of usefully factorized representation learning.

==> 1_v2_introduction.tex <==
\section{Introduction}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/cover3.pdf}
    \caption{Illustration of three learned potential landscapes $u^1$, $u^2$, $u^3$ (colored surfaces), the gradient-flow induced latent trajectories $\vz_1, \ldots, \vz_4$ (red), and the resulting decoded transforming MNIST observations. We see that each potential function has learned to model a distinct ground truth transformation, effectively factorizing the latent space at each point into a set of distinct flows.
\mw{I am not sure this figure describes what we want to convey: I think one surface with different directions on it corresponding to different transformation would do more justice to the idea}    }
    \label{fig:cover}
\end{figure}

\begin{itemize}
\item \textbf{The optimal structure for a learned representation is still unknown}
\begin{itemize}
\item Developing models which learn useful representations of data has become an increasingly important focus in the machine learning community.
\item For example, Large Language Models such as GPT~\cite{brown2020language} rely on an extensive pre-training phase to learn valuable representations, enabling quick finetuning on a diversity of tasks.
\item However, a precise definition of what makes an ideal representation is still debated.
\end{itemize}

\item \textbf{Disentanglement is one approach, but it is ill-specified.}
\begin{itemize}
\item One line of work has focused on ‘disentanglement’ of the underlying ground truth generative factors.
\item Many precise definitions have been proposed to describe this, including \mw{statistically independent factors of variation} axis-aligned single-dimensional manipulation~\cite{higgins2016beta,chen2016infogan}, linear multi-dimensional traversals~\cite{song2022orthogonal,shen2021closed,wei2021orthogonal,peebles2020hessian}, and more recently dynamic non-linear vector-based traversals~\cite{Tzelepis_2021_ICCV,song2023latent}.
\item Although these methods have been met with significant success (and even linked to single neuron brain activity), there are known theoretical limitations which make them ill-specified, including the presence of topological defects.
% \item Furthermore, these methods are empirically rather than theoretically derived
\item This has limited their deployment beyond toy settings.
\end{itemize}


\item \textbf{Equivariance is another possibility, but it is restrictive.}
\begin{itemize}
\item Another line of work has focused on developing representations which respect symmetries of the underlying data in their output space. \mw{cite Cohen et al and later work by Higgins et al}

\item Specifically, equivariant representations are those for which the output transforms in a known predictable way for a given input transformation.

\item It can be viewed as similar to disentanglement since an object undergoing a transformation which preserves its identity can be called a symmetry transformation. 
Equivariant networks however are much more strictly defined than disentanglement methods, allowing for significantly greater control and theoretical guarantees with respect to the learned transformation, however this precision also limits the types of transformations to which they may be applied.
\item For example, currently only group transformations are supported, limiting real-world applicability.
\end{itemize}

\item \textbf{Flow Factorization is more flexible, composable, generalizable, and approximately equivariant.}
\begin{itemize}
\item In this work, we provide an alternative viewpoint at the intersection of these two fields of work which we call Flow Factorized Representation Learning.
Specifically, we outline a more flexible definition for structured representation learning which still maintains many of the beneficial properties of disentangled and equivariant representations.
\item For example, we demonstrate empirically that our representations are usefully factorized, allowing flexible composability, and generalization to new datasets. 
\item Furthermore, we show that our methods are also approximately equivariant by demonstrating that they commute with input transformations through learned latent flows. 
\item Ultimately, we see these factors combined to yield the highest likelihood on the test set in each setting. 
\end{itemize}
\end{itemize}






==> 3_method.tex <==
%\section{Equivariant VAEs through Fluid Mechanical Traversal}

%\subsection{Fluid Mechanical Optimal Transport}


%\subsection{Equivariant VAEs}
\section{The Generative Model}

% \ak{I think we should reorder this section to first introduce the generative model as a whole, including k for the supervised case as an observed R.V., and the diffusion prior. We can then introduce the posterior flow and connection to OT to describe our variational approximation to the posterior.}

% \ak{Generative Model -- $p(\bar{\vx}, \bar{\vz}, k) = p(k)p(\vz_0)p(\vx_0|\vz_0) \prod_{t=1}^T p(\vz_t | \vz_{t-1}, k) p(\vx_t | \vz_t) $}

% \ak{What is $p(\vz_{t} | \vz_{t-1})$? can we derive it with the continuous change of variables?}

% \ak{Approximate Posterior (weakly sup.) -- $ q( \bar{\vz}, k | \bar{\vx}) = q(k | \bar{\vx}) q(\vz_0 | \vx_0)  \prod_{t=1}^T q(\vz_t | \vz_{t-1}, k)$}

% \ak{Approximate Posterior (Observed k) -- $ q( \bar{\vz} | \bar{\vx}, k) =  q(\vz_0 | \vx_0)  \prod_{t=1}^T q(\vz_t | \vz_{t-1}, k)$}

% \ak{$q($}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.99\linewidth]{imgs/overview.pdf}
%     \caption{Overview of our probabilistic framework for modeling sequences of image transformations. }
%     \label{fig:overview}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.99\linewidth]{imgs/graphical_model.png}
    \caption{Depiction of our model in plate notation. (Left) Supervised, (Right) Weakly-supervised. White nodes denote latent variables, shaded nodes denote observed variables, solid lines denote the generative model while dashed lines denote the approximate posterior. We see, as in a standard variational autoencoder, our model approximates the initial one-step posterior $p(\vz_0 | \vx_0)$, but additionally approximates the conditional transition distribution $p(\vz_{t}|\vz_{t-1}, k)$ through optimal transport over an approximate potential landscape.}
    \label{fig:overview}
\end{figure}


In this section we first introduce our generative model of sequences before then describing how we perform inference over the latent variables of this model. 

\subsection{Flow Factorized Sequence Distributions}
The model in this work defines a distribution over sequences of observed variables. It further factorizes this distribution into $k$ distinct components by assuming that each observed sequence is generated by one of $k$ separate flows of probability mass in latent space. Since in this work  we model discrete sequences of observations $\bar{\vx} = \{\vx_0, \vx_1 \ldots, \vx_T\}$, we aim to find a joint likelihood with a similarly discrete sequences of latent variables $\bar{\vz} = \{\vz_0, \vz_1 \ldots, \vz_T\}$, and a categorical latent variable $k$ describing the sequence type. Explicitly, we assert the following factorization of the joint likelihood over $T$ timesteps:
\begin{equation}
p(\bar{\vx}, \bar{\vz}, k) = p(k)p(\vz_0)p(\vx_0|\vz_0) \prod_{t=1}^T p(\vz_t | \vz_{t-1}, k) p(\vx_t | \vz_t).    
\end{equation}
Here $p(k)$ is a categorical distribution defining the transformation type, $p(\vx_t|\vz_t)$ asserts a mapping from latents to observations with Gaussian noise, and $p(\vz_0) = \mathcal{N}(0, 1)$. A plate diagram of this model is depicted through the solid lines in Figure \ref{fig:overview}.

To enforce that the time dynamics of the sequence define a proper flow of probability density, we compute the conditional update $p(\vz_t | \vz_{t-1}, k)$ from the continuous form of the continuity equation: $\partial_t p(\vz) = - \nabla \cdot (p(\vz) \nabla \phi^k(\vz))$, where $\phi^k(\vz)$ is the $k$'th potential function which advects the density $p(\vz)$ through the induced velocity field $\nabla \phi^k(\vz)$.
Considering the discrete particle evolution corresponding to this density evolution, $\vz_t = f(\vz_{t-1}, k) = \vz_{t-1} + \nabla_z \phi^k(\vz_{t-1})$, we see that we can derive the conditional update from the continuous change of variables formula \cite{chen2019neural}: 
\begin{equation}
p(\vz_t | \vz_{t-1}, k)  = p(\vz_{t-1}) \Big|\frac{\mathop{d f(\vz_{t-1}, k)}}{\mathop{d\vz_{t-1}}}\Big|^{-1}
\end{equation}
% $ = -p(\vz_{t-1}) | 1 + \nabla^2_z \phi^k(\vz_{t-1})|
% From Theorem 2.1 of \cite{neklyudov2023action}, we know that `under mild conditions ... any continuous dynamics can be modeled by the continuity equation', for some function $\phi^*$, and thus conclude that this framework has sufficient capability to model a diversity of continuous latent dynamics.
% \subsection{Diffusion prior evolution} 
In this setting, we see that the choice of $\phi$ ultimately determines the prior on the transition probability in our model. As a minimally informative prior for random trajectories, we use a diffusion equation achieved by simply taking $\psi^k=-D_k\log p(\vz_t)$. Then according to the continuity equation, the prior  evolves as:
\begin{equation}
    \partial_t p(\vz_t) = -\nabla\cdot\Big(p(\vz_t)\nabla\psi\Big)= D_k\nabla^2  p(\vz_t)
\end{equation}
where $D_k$ is a constant coefficient that does not change over time. The density evolution of the prior distribution thus follows the constant diffusion process. We set $D^k$ as a learnable parameter which is distinct for each $k$.

\subsection{Inference}


\subsection{}



\section{Methodology}

% \ak{I think we should reorder this section to first introduce the generative model as a whole, including k for the supervised case as an observed R.V., and the diffusion prior. We can then introduce the posterior flow and connection to OT to describe our variational approximation to the posterior.}

% \ak{Generative Model -- $p(\bar{\vx}, \bar{\vz}, k) = p(k)p(\vz_0)p(\vx_0|\vz_0) \prod_{t=1}^T p(\vz_t | \vz_{t-1}, k) p(\vx_t | \vz_t) $}

% \ak{Approximate Posterior (weakly sup.) -- $ q( \bar{\vz}, k | \bar{\vx}) = q(k | \bar{\vx}) q(\vz_0 | \vx_0)  \prod_{t=1}^T q(\vz_t | \vz_{t-1}, k)$}

% \ak{Approximate Posterior (Observed k) -- $ q( \bar{\vz} | \bar{\vx}, k) =  q(\vz_0 | \vx_0)  \prod_{t=1}^T q(\vz_t | \vz_{t-1}, k)$}

% \textbf{Time Conditional: $p(\vz_t | \vz_{t-1}, k)$}
% \begin{itemize}
%     \item The last part of our generative model to define is the time-evolution through the conditional $p(\vz_t | \vz_{t-1}, k)$. We see that $\vz_t$ is determined not only by the previous timestep, but also by the sequence category variable $k$.
%     \item 
    
%     \item We choose to derive our choice of prior by first starting in continuous time, defining $\partial_t p(\vz|k)$, from which we can use the change of variables to obtain the discrete version.
%     \item In particular, we let  $\partial_t p(\vz) = -\nabla\cdot\Big(p(\vz)\nabla\psi\Big)= D\nabla^2  p(\vz)$

%     \item \textbf{Discrete Time}
    
% \end{itemize}



Fig.~\ref{fig:overview} depicts the overview of our method. We train our VAE to learn $K$ different image sequences $\vx_0 \rightarrow \vx_T$ by moving the latent code of the initial image $\vz_0$ through $K$ velocity fields $\nabla u^k$. The specific image transformation is randomly sampled at each iteration. The potential $u^k(\vz_, t) = \texttt{MLP}([\vz;t])$ defines the scalar time-dependent potential function for the $k$-th transformation. Its gradient field $\nabla_\vz u^k$ pushes the initial posterior distribution to the target distribution via dynamic OT. For the prior distribution, we assume it is Markov and explicitly use a constant diffusion equation for modeling the random evolution. When the transformation index $k$ is not available, another encoder is embraced in our framework to predict the one-hot index. In the following, we elaborate on each component of our framework in detail.

%Depending on the supervision setting, the transformation index $k$ can be either available or not. The latent code evolves following a velocity field as $\vz_{t} = \vz_{t-1} + \nabla_\vz u^k(\vz_{t-1}, t-1)$ where $u^k(\vz_{t}, t) = \texttt{MLP}([\vz_t;t])$ defines the scalar time-dependent potential function for $k$-th transformation. The gradient field $\nabla_\vz u^k$ pushes the initial posterior distribution to the target distribution via dynamic optimal transport, while the prior distribution follows the constant diffusion process. In the following, we elaborate on each component of our framework in detail.

\subsection{Sequence model}

We consider our VAE as a sequence model and we would like to maximize the Evidence Lower BOund (ELBO) of the joint probability of the sequence  $p(\vx_0, \vx_1, \ldots, \vx_T)$. For simplicity, we use $\bar{\vx}$ and $\bar{\vz}$ to represent the sequence $\vx_{0},\dots,\vx_{T}$ and $\vz_{0},\dots,\vz_{T}$, respectively. Our goal is to optimize:
\begin{equation}
\begin{aligned}
\log p(\bar{\vx})&= \E_{q_{\theta}(\bar{\vz}|\bar{\vx})} \left[ \log\frac{p(\bar{\vx},\bar{\vz})}{q(\bar{\vz}|\bar{\vx})}\frac{q(\bar{\vz}|\bar{\vx})}{p(\bar{\vz}|\bar{\vx})}\right]\\
&\geq \E_{q_{\theta}(\bar{\vz}|\bar{\vx})} \left[ \log\frac{p(\bar{\vx}|\bar{\vz})p(\bar{\vz})}{q(\bar{\vz}|\bar{\vx})}\right]\\
&=\E_{q_{\theta}(\bar{\vz}|\bar{\vx})} \left[ \log p(\bar{\vx}|\bar{\vz})\right] + \E_{q_{\theta}(\bar{\vz}|\bar{\vx})} \left[\log\frac{p(\bar{\vz})}{q(\bar{\vz}|\bar{\vx})}\right]
\end{aligned}
\label{eq:joint_prob}
\end{equation}
In our case, all the future latent codes $\vz_t$ are attained by moving the initial sample $\vz_0$ and thus only conditioned on $\vx_0$. It is sufficient to change the definition of the posterior from $q(\bar{\vz}|\bar{\vx})$ to $q(\bar{\vz}|\vx_0)$. We assume that the posterior distributions of each element are independent and the priors follow the Markov decision process. That is:
\begin{equation}
    \begin{split}
        q(\bar{\vz}|\vx_0) = q(\vz_{0}|\vx_{0})q(\vz_{1}|\vx_{0})\dots q(\vz_{T}|\vx_{0}),\ p(\hat{\vz}) = p(\vz_0)p(\vz_{1}|\vz_0)\dots p(\vz_{T}|\vz_{T-1})
    \end{split}
\label{eq:assumption}
\end{equation}
Under the assumptions, Eq.~(\ref{eq:joint_prob}) can be re-written as:
\begin{equation}
    \begin{aligned}
    \log p(\bar{\vx})&\geq \sum_{t=0}^{T}\E_{q_{\theta}(\vz_{t}|\vx_{0})} \big[ \log p(\vx_{t}|\vz_{t}) - \mathrm{D}_{\text{KL}}\left[ q_{\theta}(\vz_{t}|\vx_{0}, k) || p(\vz_{t} | \vz_{t-1}, k) \right] \big] = \sum_{t=0}^{T}\log p(\vx_t)
    \end{aligned}
\end{equation}
This turns the original optimization objective into maximizing the probability of each element in the sequence. Now we proceed to introduce how the latent code $\vz_t$ evolves during the traversal.   




%\noindent\textbf{Evidence Lower Bound.}

%\subsection{HJ Equation as Velocity Fields}
\subsection{Dynamic optimal latent traversal}

We use the gradient of the potential function $u^k(\vz,t)$ to move the latent code as $\vz_t = \vz_{t-1} + \nabla u^k$. Since OT can  move the distribution to the target via the shortest path, we assume the OT is an efficient way for learning disentangled representations. The spatial-temporal dynamics of the latent traversal naturally link to the fluid mechanical dynamic interpretation of OT: when the velocity field $\nabla u^k$ satisfies certain PDEs, the evolution can be seen to minimize the Wasserstein distance between the source and target distributions. Specifically, we have the following theorem:

\begin{thm}[Benamou-Brenier Formula~\cite{benamou2000computational}]
For probability measures $\mu_{0}$ and $\mu_{1}$, the $L_{2}$ Wasserstein distance can be defined as
\begin{equation}
     W_2(\mu_{0},\mu_{1}) = \min \{\sqrt{\int\int \frac{1}{2}\rho(x,t)|v(x,t)|^2\mathop{dx}\mathop{dt}} \}
\end{equation}
 where the density $\rho$ and the velocity $v$ satisfy:
\begin{equation}
     \frac{\mathop{d}\rho(x,t)}{\mathop{dt}} = -\nabla\cdot(v(x,t)\rho(x,t)),\ v(x,t)=\nabla\phi(x,t)
 \end{equation}
% and the potential $\phi$ satisfies the Hamilton-Jacobi equation:
% \begin{equation}
%      \frac{\mathop{d}\phi(x,t)}{\mathop{dt}} + \frac{1}{2}|\nabla\phi(x,t)|^2 =0
%\end{equation}
\end{thm}
The optimality condition of the velocity is given by the generalized Hamilton-Jacobi (HJ) equation (\emph{i.e.,} $\partial_t \phi + \nicefrac{1}{2}||\nabla\phi||^2\leq 0$). The detailed derivation is deferred to the supplementary. We thus encourage our potential energy to satisfy the HJ equation with an external driving force as
\begin{equation}
   \frac{\partial}{\partial t} u^{k}(\vz,t)+ \frac{1}{2} ||\nabla_\vz u^{k}(\vz,t)||^2 = f(\vz,t)\ subject\ to\ f(\vz,t)\leq0 
\end{equation}  
Here we use another \texttt{MLP} to parameterize the external force $f(\vz,t)$ and realize the negativity constraint by setting $f(\vz,t)=-\texttt{MLP}([\vz;t])^2$. To achieve the PDE constraint, we impose a Physics-Informed Neural Network (PINN)~\cite{pinns} loss as
\begin{equation}
    \gL_{HJ}=\frac{1}{T}\sum_{t=1}^T \Big(\frac{\partial}{\partial t} u^{k}(\vz,t)+ \frac{1}{2} ||\nabla_\vz u^{k}(\vz,t)||^2-f(\vz,t)\Big)^2 + ||\nabla u^k (\vz_0,0)||^2
\end{equation}
where the first term restricts the potential obeys the HJ equation, and the second term limits $u(\vz_t, t)$ to return no update at $t{=}0$, therefore matching the initial condition.


%\noindent\textbf{Potential Flows}
\subsection{Flow-like posterior evolution}

%The latent sample motion corresponds to an equivalent evolution in the density space. 
By the formula of change of variables, the sample evolution would have the corresponding equivalent evolution in the density. Given the function of the sample evolution $\vz_{t}=g(\vz_{t-1})=\vz_{t-1} + \nabla_{\vz} u^k$, the law of conservation of mass $\int q(\vz_{t}|\vx_0) \mathop{d\vz_{t}} =  \int q(\vz_{t-1}|\vx_{0})\mathop{d\vz_{t-1}}$ gives:
\begin{equation}
    q(\vz_{t}|\vx_0)=q(\vz_{t-1}|\vx_{0})\Big|\frac{\mathop{d\vz_{t-1}}}{\mathop{d\vz_{t}} }\Big| = q(\vz_{t-1}|\vx_{0})\Big|\frac{\mathop{dg(\vz_{t-1})}}{\mathop{d\vz_{t-1}} }\Big|^{-1}
\end{equation}
Discretizing the latent codes and taking the logarithm of both sides gives the normalizing-flow-like density evolution of our posterior:
\begin{equation}
     \log q(\vz_{t}|\vx_0) = \log  q(\vz_{t-1}|\vx_{0}) - \log |1+\nabla_{\vz}^2 u^k|
\end{equation}
%The latent sample is evolved following the function $\vz_{t}=g(\vz_{t-1})=\vz_{t-1} + \nabla_{\vz}u$, which has an equivalent representation in the density evolution. 
The above relation can be equivalently derived from the continuity equation (\emph{i.e.,} $\partial_t q(\vz_t|\vx_0) = -\nabla\cdot\big(q(\vz_t|\vx_0)\nabla u\big)$). Notice that we only assume the initial posterior $q(\vz_0|\vx_0)$ follows a Gaussian distribution. For future timesteps, we do not pose any further assumption and just let the density evolves according to the sample motion.

%Normalizing flow-like evolution of the density.

% \subsection{Diffusion prior evolution} 

% As shown in Eq.~(\ref{eq:assumption}), due to the flow-like evolution (\emph{i.e.,} the current states depends on the previous one), we assume the priors follow the properties of the Markov chain. One particularly suitable PDE for modeling such Markov chains is the diffusion equation. Since there is no a priori knowledge about the image transformation of the sequence, we use diffusion equations to model the behavior as random particle movements. Different from the posterior evolution that use parametric \texttt{MLPs}, we simply take $\psi=-D\log p(\vz_t)$ and use $\nabla\psi=\nicefrac{-D\nabla p(\vz_t)}{p(\vz_t)}$ as the velocity field. Then according to the continuity equation, the prior would evolve as
% \begin{equation}
%     \partial_t p(\vz_t) = -\nabla\cdot\Big(p(\vz_t)\nabla\psi\Big)= D\nabla^2  p(\vz_t)
% \end{equation}
% where $D$ is a constant coefficient that does not change over time. The density evolution of the prior distribution thus follows the constant diffusion process. We set $D$ as a learnable parameter and use different $D$ for different transformations.


%which is often used to describe the particle behavior in Brownian motion

\subsection{Weakly-supervised setting}

We also consider the weakly supervised setting of our method where we are given different image sequences $\bar\vx$ but have no access to the transformation index $k$. In this setting, we use an extra encoder/posterior $q_{\gamma}(k|\bar\vx)$ and integrate it into the ELBO framework. With the relation $p(\bar{\vx},\bar{\vz},k)=p(\bar{\vx})p(k|\bar{\vx})p(\bar{\vz}|\bar{\vx},k)$, Bayes' theorem gives:
\begin{equation}
    p(\bar{\vx})=\frac{p(\bar{\vx},\bar{\vz},k)}{p(k|\bar{\vx})p(\bar{\vz}|\bar{\vx},k)}=\frac{p(\bar{\vx},\bar{\vz}|k)}{p(\bar{\vz}|\bar{\vx},k)}\frac{p(k)}{p(k|\bar{\vx})}
\end{equation}
Then the new ELBO can be re-formulated as
\begin{equation}
    \begin{aligned}
\log p(\bar{\vx})&= \E_{q_{\theta}(\bar{\vz}|\bar{\vx},k),q_{\gamma}(k|\bar{\vx})} \left[ \log
\frac{p(\bar{\vx},\bar{\vz}|k)}{q(\bar{\vz}|\bar{\vx},k)}
\frac{q(\bar{\vz}|\bar{\vx},k)}{p(\bar{\vz}|\bar{\vx},k)}
\frac{p(k)}{q(k|\bar{\vx})}
\frac{q(k|\bar{\vx})}{p(k|\bar{\vx})}\right]\\
&\geq\E_{q_{\theta}(\bar{\vz}|\bar{\vx},k),q_{\gamma}(k|\bar{\vx})} \left[ \log\frac{p(\bar{\vx}|\bar{\vz},k)p(\bar{\vz}|k)}{q(\bar{\vz}|\bar{\vx},k)}\frac{p(k)}{q(k|\bar{\vx})}\right]\\
&=\E_{q_{\theta}(\bar{\vz}|\bar{\vx},k)} \left[ \log p(\bar{\vx}|\bar{\vz},k)\right] + \E_{q_{\theta}(\bar{\vz}|\bar{\vx},k)} \left[\log\frac{p(\bar{\vz}|k)}{q(\bar{\vz}|\bar{\vx},k)} \right] + \E_{q_{\gamma}(k|\bar{\vx})} \left[\log\frac{p(k)}{q(k|\bar{\vx})} \right]\\
%&=\sum_{t=0}^{T}\E_{q_{\theta}(\vz_{t}|\vx_{t},k)} \big[ \log p(\vz_{t}|\vx_{t},k) - \mathrm{D}_{\text{KL}}\left[ q_{\theta}(\vz_{t}|\vx_{t},k) || p(\vz_{t}|k) \right] \big] -\E_{q_{\gamma}(k|\bar{\vx})}\big[\mathrm{D}_{\text{KL}}\left[q(k|\bar{\vx})|p(k)\right]\big]
\end{aligned}
\end{equation}
It turns out that compared with Eq.~(\ref{eq:joint_prob}), only one additional KL divergence $ \mathrm{D}_{\text{KL}}\left[ q_{\gamma}(k|\bar\vx) || p(k) \right] \big]$ is needed to compensate for the index supervision. The prior $p(k)$ is set to follow a categorical distribution, and we apply the \texttt{Gumbel-SoftMax} trick~\cite{jang2017categorical} to allow for categorical re-parameterization and sampling of $q_{\gamma}(k|\bar\vx)$.

